SHARP: Shielding-Aware Robust Planning for Safe and Efficient Human-Robot Interaction

Jointly achieving safety and efficiency in human-robot interaction (HRI) settings is a challenging problem, as the robot's planning objectives may be at odds with the human's own intent and expectations. Recent approaches ensure safe robot operation in uncertain environments through a supervisory control scheme, sometimes called "shielding", which overrides the robot's nominal plan with a safety fallback strategy when a safety-critical event is imminent. These reactive "last-resort" strategies (typically in the form of aggressive emergency maneuvers) focus on preserving safety without efficiency considerations; when the nominal planner is unaware of possible safety overrides, shielding can be activated more frequently than necessary, leading to degraded performance. In this work, we propose a new shielding-based planning approach that allows the robot to plan efficiently by explicitly accounting for possible future shielding events. Leveraging recent work on Bayesian human motion prediction, the resulting robot policy proactively balances nominal performance with the risk of high-cost emergency maneuvers triggered by low-probability human behaviors. We formalize Shielding-Aware Robust Planning (SHARP) as a stochastic optimal control problem and propose a computationally efficient framework for finding tractable approximate solutions at runtime. Our method outperforms the shielding-agnostic motion planning baseline (equipped with the same human intent inference scheme) on simulated driving examples with human trajectories taken from the recently released Waymo Open Motion Dataset.

==> notation.tex <==
% !TeX root = thesis.tex

% This file contains the notation macros for the entire paper.


% ----------- LaTeX Environments -----------

\usepackage{amsthm}  % Ensure we are using amsthm.
\usepackage{amsmath}
\usepackage{bm}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}

\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

\newtheorem{remark}{Remark}

\newtheorem*{example}{Illustrative Example}

\usepackage{ifthen}
\newboolean{include-notes}
\setboolean{include-notes}{false}  % Set boolean to false to hide all notes and "to-be-removed" text.

\usepackage{xcolor}
\newcommand{\jaime}[1]{\ifthenelse{\boolean{include-notes}}{\textcolor{orange}{\textbf{Jaime:} #1}}{}}
\newcommand{\haimin}[1]{\ifthenelse{\boolean{include-notes}}{\textcolor{teal}{\textbf{Haimin:} #1}}{}}
\newcommand{\remove}[1]{\ifthenelse{\boolean{include-notes}}{\textcolor{red}{\sout{#1}}}{}}
\newcommand{\new}[1]{\ifthenelse{\boolean{include-notes}}{\textcolor{magenta}{#1}}{#1}}

%%%%%%%%%%

\usepackage{lipsum}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
%%%%%%

    
% \newcommand{\example}[1]%
% {
% \textbf{Running example:}
% \textit{#1}
% }

% ---------------- Notation ----------------

% Sets and spaces

\newcommand{\reals}{\mathbb{R}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\integers}{\mathbbb{Z}}
\newcommand{\compl}{\mathsf{c}}
\newcommand{\bdry}{{\partial}}
\newcommand{\ball}{{B}}
\newcommand{\radius}{{r}}


% Dynamical system

\newcommand{\iagent}{{i}}
\newcommand{\nagents}{{N}}
\newcommand{\iagentset}{{\mathcal{I}}}
\newcommand{\iagentbis}{{j}}
\newcommand{\iagentaux}{{k}}

\newcommand{\state}{{x}}
\newcommand{\ctrl}{{u}}
\newcommand{\dstb}{{d}}
\newcommand{\costate}{{p}}
\newcommand{\traj}{{\mathbf{x}}}%{{\xi}}%
\newcommand{\ctrlsig}{{\mathbf{u}}}
\newcommand{\dstbsig}{{\mathbf{d}}}
\newcommand{\stateaux}{{\tilde{\state}}}
\newcommand{\stateinit}{{\state_0}}
\newcommand{\statebis}{{z}}

\newcommand{\stateset}{{\mathcal{C}}}  %{{\reals^\nx}}
\newcommand{\ctrlset}{{\mathcal{U}}}
\newcommand{\dstbset}{{\mathcal{D}}}
\newcommand{\trajset}{{\mathbb{X}}}
\newcommand{\csigset}{{\mathbb{U}}}
\newcommand{\dsigset}{{\mathbb{D}}}
\newcommand{\xsetbis}{{\reals^\naux}}
\newcommand{\wspace}{{\mathcal{W}}}  % workspace

% \newcommand{\nx}{{n}}
% \newcommand{\nc}{{n_\ctrl}}
% \newcommand{\nd}{{n_\dstb}}
% \newcommand{\nci}{{n_{\ctrl_\iagent}}}
% \newcommand{\naux}{{m}}

% \newcommand{\xsubset}{{\mathcal{X}}}
% \newcommand{\hatD}{{\hat{\dset}}}
% \newcommand{\hatDx}{{\hatD(\state)}}

\newcommand{\dyn}{{f}}
% \newcommand{\dynset}{{F}}
% \newcommand{\dynstate}{{\dyn_\state}}
% \newcommand{\dyndstb}{{\dyn_\dstb}}
% \newcommand{\dyntrue}{{\dyn^*}}

% \newcommand{\tcont}{{t}}
% \newcommand{\tdisc}{{k}}
% \newcommand{\tstep}{{\delta}}
% \newcommand{\tstart}{{\tcont_0}}
% \newcommand{\tend}{{\tcont_f}}
% \newcommand{\thorizon}{{T}}
% \newcommand{\khorizon}{{K}}
% \newcommand{\tcontaux}{{\tau}}
% \newcommand{\tcontbis}{{s}}
% \newcommand{\tdiscaux}{{l}}
% \newcommand{\tdiscstart}{{\tdisc_0}}

% \newcommand{\xdisc}{{\state_\mathbf{i}}}
% \newcommand{\udisc}{{\ctrl_\mathbf{j}}}
% \newcommand{\Xdisc}{{\mathbf{X}}}
% \newcommand{\Udisc}{{\mathbf{U}}}
% \newcommand{\fdisc}{{\mathbf{f}}}


% Optimal control and dynamic games

\newcommand{\outcome}{{\mathcal{V}}}
\newcommand{\valfunc}{{V}}
\newcommand{\qfunc}{{Q}}

\newcommand{\policy}{{\pi}}
\newcommand{\strat}{{\gamma}}
\newcommand{\cstrat}{{\bm{\upsilon}}}
\newcommand{\dstrat}{{\bm{\delta}}}

% \newcommand{\policyset}{{\Pi}}
% \newcommand{\cstratset}{{\mathfrak{U}}}
% \newcommand{\dstratset}{{\mathfrak{D}}}

% \newcommand{\surffunc}{{\psi}}
% \newcommand{\distfunc}{s}
% \newcommand{\consfunc}{{g}}
% \newcommand{\targfunc}{{l}}
% \newcommand{\costfunc}{{c}}
% \newcommand{\mayerterm}{{M}}
% \newcommand{\lagrangian}{{L}}
% \newcommand{\hamiltonian}{{H}}
% \newcommand{\HJparticle}{{\Lambda}}

% \newcommand{\dmap}{{\phi}}


% Safety analysis

\newcommand{\safeset}{{\Omega}}
\newcommand{\levelset}{{\mathcal{Q}}}

\newcommand{\set}{{\mathcal{M}}}
\newcommand{\target}{{\mathcal{T}}}
\newcommand{\constraint}{{\mathcal{K}}}
\newcommand{\failure}{{\mathcal{F}}}
\newcommand{\reach}{{\mathcal{R}}}
\newcommand{\reachinev}{{\underline\reach}}
\newcommand{\reachrbst}{{\overline\reach}}
\newcommand{\reachavoid}{{\mathcal{RA}}}
\newcommand{\reachavoidinev}{{\underline\reachavoid}}
\newcommand{\reachavoidrbst}{{\overline\reachavoid}}
\newcommand{\reachavoidDiscount}{{\reachavoid_\gamma}}
\newcommand{\inv}{{\text{\textnormal{Inv}}}}
\newcommand{\viab}{{\text{\textnormal{Viab}}}}
\newcommand{\disc}{{\text{\textnormal{Disc}}}}

\newcommand{\frs}{{\overrightarrow{\reach}}}
\newcommand{\brs}{{\overleftarrow{\reach}}}
\newcommand{\fras}{{\overrightarrow{\reachavoid}}}
\newcommand{\bras}{{\overleftarrow{\reachavoid}}}

\newcommand{\hidden}{{\mathcal{H}}}
\newcommand{\obj}{{\tilde{o}}}
\newcommand{\obst}{{\mathcal{O}}}
\newcommand{\capture}{{\text{Cap}}}
\newcommand{\capturebasin}{{\mathcal{B}}}
\newcommand{\fhs}{{\overrightarrow{\hidden}}}



\newcommand{\tset}{{\mathbb{M}}}
\newcommand{\ttarget}{{\mathbb{T}}}
\newcommand{\tconstraint}{{\mathbb{K}}}
\newcommand{\tfailure}{{\mathbb{F}}}
\newcommand{\treachavoid}{{\mathbb{RA}}}
\newcommand{\treachavoidinev}{{\underline\treachavoid}}
\newcommand{\treachavoidrbst}{{\overline\treachavoid}}


% Probability

% \newcommand{\prob}{{P}}
% \newcommand{\gaussian}{{\mathcal{N}}}
% \newcommand{\gp}{{\mathcal{GP}}}
% \newcommand{\probd}{{\prob_\dstb}}
% \newcommand{\probx}{{\prob_\state}}
% \newcommand{\probtraj}{{\prob_\traj}}


% Calculus

\newcommand{\grad}{{\nabla}}
\newcommand{\totalderiv}{{D}}


% Quadrotor flight
% \newcommand{\altitude}{{h}}


% Datasets

% \newcommand{\xdata}{{X}}
% \newcommand{\ddata}{{D}}


% Operators

\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\cov}{cov}


% Trajectory Planning
\newcommand{\pos}{{p}} % position
% \newcommand{\npos}{{\nx_\pos}} % position
% \newcommand{\postraj}{{\mathbf{\pos}}} %position trajectory
% \newcommand{\captradius}{{R_c}} % Capture radius
% \newcommand{\captside}{{L_c}} % Capture side (for box)

% \newcommand{\posx}{{\textnormal{x}}}
% \newcommand{\posy}{{\textnormal{y}}}
% \newcommand{\posz}{{\textnormal{z}}}
% \newcommand{\vel}{{v}} % velocity
% \newcommand{\yaw}{{\psi}}
% \newcommand{\roll}{{\phi}}
% \newcommand{\pitch}{{\theta}}
% \newcommand{\angvel}{{\omega}}
% \newcommand{\thrust}{{\tau}}
% \newcommand{\grav}{{g}}
% \newcommand{\acc}{{a}}

% \newcommand{\etd}{\tcont^{0-}} % earliest time of departure
% \newcommand{\ltd}{\tcont^{0+}} % latest time of departure
% \newcommand{\sta}{\thorizon}%{\tcont^\text{STA}} % scheduled time of arrival

\newcommand{\danger}{{\mathcal{D}}} % Danger (failure) zone in joint state space
% \newcommand{\iobst}{{\mathcal{O}}} % Induced obstacle in position space
% \newcommand{\ifail}{{\failure}} % Induced obstacle
% \newcommand{\sfail}{\failure^0} % static obstacle in state space
% \newcommand{\wcttr}{\tcont^\text{WC}} % worst case TTR


% Robust Trajectory Planning
% \newcommand{\errorbound}{{\mathcal{E}}}
% \newcommand{\erradius}{R^\errorbound}
% \newcommand{\error}{{e}}
% \newcommand{\transform}{{\phi}}
% \newcommand{\errortraj}{{\mathbf{\error}}}

% \newcommand{\trajnom}{\traj^p}
% \newcommand{\statenom}{\state^p}
% \newcommand{\posnom}{\pos^p}
% \newcommand{\posxnom}{\posx^p}
% \newcommand{\posynom}{\posy^p}
% \newcommand{\posznom}{\posz^p}
% \newcommand{\yawnom}{\yaw^p}
% \newcommand{\velnom}{\vel^p}
% \newcommand{\angvelnom}{\angvel^p}
% \newcommand{\ctrlnom}{\ctrl^p}
% \newcommand{\csetnom}{\cset^p}
% \newcommand{\csignom}{\csig^p}
% \newcommand{\csigsetnom}{\csigset^p}
% \newcommand{\cstratnom}{\cstrat^p}
% \newcommand{\cstratsetnom}{\cstratset^p}

% \newcommand{\xrbst}{{\tilde{\xsubset}}} % roubst tracking set
% \newcommand{\targrbst}{{\tilde{\target}}}
% \newcommand{\failrbst}{{\tilde{\failure}}}
% \newcommand{\tfailrbst}{{\tilde{\tfailure}}}
% \newcommand{\ifailrbst}{{\tilde{\ifail}}}
% \newcommand{\iobstrbst}{{\tilde{\iobst}}}



% FaSTrack + Human-Robot Systems
% \newcommand{\tstate}{\state}    % Tracker state
% \newcommand{\pstate}{\state^p}  % Planner state
% \newcommand{\rstate}{\error}    % Error state
% \newcommand{\nt}{\nx}           % Tracker state dimension
% \newcommand{\np}{\nx^p}         % Planner state dimension
% \newcommand{\txset}{\reals^{\nt}}       % {\mathcal{X}} %tracker set
% \newcommand{\pxset}{\reals^{\np}}       % {\mathcal{S}} %planner set

% \newcommand{\ttraj}{\traj}              % Tracker trajectory
% \newcommand{\ptraj}{\traj^{p}}          % Planner trajectory
% \newcommand{\rtraj}{\mathbf{\error}}    % Error trajectory

% \newcommand{\tctrl}{\ctrl}      % Tracker control
% \newcommand{\pctrl}{\ctrl^p}    % Planner control
% \newcommand{\tcset}{\cset}      % Tracker control set
% \newcommand{\pcset}{\cset^p}    % Tracker control set

% \newcommand{\tdyn}{\dyn}       % Tracker dynamics
% \newcommand{\pdyn}{\dyn^p}     % Planner dynamics
% \newcommand{\rdyn}{\dyn^e}     % Relative dynamics

% \newcommand{\reward}{\lagrangian}       % Reward function
\newcommand{\footprint}{{\phi}}    % Robot footprint (subindex for space)
% \newcommand{\tvar}{\tcont}      % Continuous time variable
% \newcommand{\thor}{\thorizon}   % Consider changing this globally

% \newcommand{\pfail}{\failure^{p}}
% \newcommand{\ptarg}{\target^{p}}
% \newcommand{\ptargrbst}{\targrbst^{p}}

\newcommand{\fov}{{\mathcal{Z}}} % Field of view (sensor)
% \newcommand{\kfrs}{\reach_F}
% \newcommand{\kbrs}{\reach_B}
% \newcommand{\frg}{\mathcal{G}_F}
% \newcommand{\brg}{\mathcal{G}_B}
% \newcommand{\env}{\mathcal{W}}
% \newcommand{\envfree}{\env_\textnormal{free}}
% \newcommand{\envgoal}{\env_\textnormal{goal}}
% \newcommand{\home}{\pstate_{\textnormal{home}}}
% \newcommand{\goal}{\pstate_{\textnormal{goal}}}
% \newcommand{\explorable}{\pxsubset_{\textnormal{SE}}}
% \newcommand{\sample}{\pstate_{\textnormal{new}}}

% \newcommand{\pxsubset}{\mathcal{P}}
% \newcommand{\freeset}{\pxsubset_{\textnormal{free}}}
% \newcommand{\goalset}{\pxsubset_{\textnormal{goal}}}


% Hierarchical Game-Theoretic Planning
\newcommand{\hstate}{{s}}
\newcommand{\hctrl}{{a}}
\newcommand{\hcset}{{\mathcal{A}}}
\newcommand{\sdyn}{{\phi}}

\newcommand{\indicator}{\ensuremath{\mathbf{1}}\xspace}
